The Life Cycle of Knowledge in Big Language Models: A Survey

Knowledge plays a critical role in artificial intelligence. Recently, the extensive success of pre-trained language models (PLMs) has raised significant attention about how knowledge can be acquired, maintained, updated and used by language models. Despite the enormous amount of related studies, there still lacks a unified view of how knowledge circulates within language models throughout the learning, tuning, and application processes, which may prevent us from further understanding the connections between current progress or realizing existing limitations. In this survey, we revisit PLMs as knowledge-based systems by dividing the life circle of knowledge in PLMs into five critical periods, and investigating how knowledge circulates when it is built, maintained and used. To this end, we systematically review existing studies of each period of the knowledge life cycle, summarize the main challenges and current limitations, and discuss future directions.

==> sections/authors.tex <==
\newpage

\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,clip,keepaspectratio]{pics/caoboxi.JPG}}
\noindent {\bf Boxi Cao}\ 
is a Ph.D. student in the Chinese Information Processing Laboratory at the Institute of Software, Chinese Academy of Sciences, under the supervision of Professor Xianpei Han and Professor Le Sun. He received Bachelor degree in Beijing University of Posts and Telecommunications in June 2019. \\
His research interest lies in natural language process, especially the knowledge in large language models, as well as information extraction. \\
Email: boxi2020@iscas.ac.cn \\
ORCID iD: 0000-0001-9916-7406
}
\vspace{1\baselineskip}


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,clip,keepaspectratio]{pics/linhongyu.jpg}}
\noindent {\bf Hongyu Lin}\ received the Ph.D. degree from the Institute of Software, Chinese Academy of Sciences, Beijing, China in 2020.
He is currently an associate professor in the institute of Software, Chinese Academy of Sciences.\\
His research interests include information extraction and knowledge mechanism in large LMs. \\
E-mail: hongyu@iscas.ac.cn
}
\vspace{1\baselineskip}


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,clip,keepaspectratio]{pics/xianpei.jpeg}}
\noindent {\bf Xianpei Han}\ 
is a professor of computer science in the CIPS Laboratory at the Institute of Software, Chinese Academy of Sciences. He received the PhD degree in Pattern Recognition and Intelligent Systems from National Laboratory of Pattern Recognition, Institute of Automation, CAS. \\
His research interests lie in natural language understanding, and has published about 60 papers  in ACL/EMNLP/SIGIR/AAAI. \\
Email: xianpei@iscas.ac.cn \\
ORCID iD: 0000-0002-1304-6302
}
\vspace{1\baselineskip}


\par\noindent 
\parbox[t]{\linewidth}{
\noindent\parpic{\includegraphics[width=1in,clip,keepaspectratio]{pics/sunle.jpg}}
\noindent {\bf Le Sun}\ 
received Ph.D. degree from Nanjing University of Science & Technology, China in 1998. He is a professor at Institute of Software, Chinese Academy of Sciences (ISCAS). He is the General Secretary of Chinese Information Processing Society of China (CIPS). He visited University of Birmingham, UK and University of Montreal, Canada as visiting scholar at 2004 and 2005. He has published more than 100 top journal and conference papers. He received the best short paper Award from SIGIR2021. In 2022, he received the Excellent Tutor Award from Chinese Academy of Sciences and First prize of Qian Weichang Chinese Information Processing Science and Technology Award. \\
His research interests lie in natural language understanding, knowledge graph, information extraction, and question answer. \\
E-mail: sunle@iscas.ac.cn
}
\vspace{1\baselineskip}





